Minimax AUC Fairness: Efficient Algorithm with Provable Convergence

The use of machine learning models in consequential decision making often exacerbates societal inequity, in particular yielding disparate impact on members of marginalized groups defined by race and gender. The area under the ROC curve (AUC) is widely used to evaluate the performance of a scoring function in machine learning, but is studied in algorithmic fairness less than other performance metrics. Due to the pairwise nature of the AUC, defining an AUC-based group fairness metric is pairwise-dependent and may involve both \emph{intra-group} and \emph{inter-group} AUCs. Importantly, considering only one category of AUCs is not sufficient to mitigate unfairness in AUC optimization. In this paper, we propose a minimax learning and bias mitigation framework that incorporates both intra-group and inter-group AUCs while maintaining utility. Based on this Rawlsian framework, we design an efficient stochastic optimization algorithm and prove its convergence to the minimum group-level AUC. We conduct numerical experiments on both synthetic and real-world datasets to validate the effectiveness of the minimax framework and the proposed optimization algorithm.

==> miscellaneous.tex <==
Given a false positive rate (FPR) range $[0, \beta]$, the partial AUC (pAUC) of $f_\theta$ is then defined as \cite{narasimhan2017support}
\[\pauc(f) = \Ebb[\Ibb[f_\theta(X) > f_\theta(X') ]\Tbb_{[0, \beta]}[f_\theta; X']| Y=+1, Y'=-1],\]
where $\Tbb_{[0, \beta]}[f_\theta; X']$ is an indicator function which is $1$ if $\Pbb[f_\theta(X'') > f_\theta(X')|Y''=-1] \in [0, \beta]$, and $0$ otherwise.

The group-level pAUC can be defined similarly as follow 
\[\pauc_{z, z'}(f) = \Ebb[\Ibb[f_\theta(X) > f_\theta(X') ]\Tbb_{[0, \beta]}[f_\theta; X', Z']| Y=+1, Y'=-1, Z=z, Z'=z'],\]
where $\Tbb_{[0, \beta]}[f_\theta; X', Z']$ is an indicator function which is $1$ if $\Pbb[f_\theta(X'') > f_\theta(X')|Y''=-1, Z''=Z'] \in [0, \beta]$, and $0$ otherwise. 

Similarly, the empirical group-level pAUC is defined as 
\[
\widehat{\pauc}_{z, z'}(f) = \widehat{\pauc}(f; S^{z+}, S^{z'-}) = \frac{1}{n^{z+} n_\beta^{z'-}}
\sum_{i=1}^{n^{z+}} \sum_{j=1}^{n_\beta^{z'-}}  \Ibb[f_\theta(\xbf_i^{z+}) > f_\theta(\xbf_{[j]}^{z'-})]
\]
where $n_\beta^{z'-} = \lceil \beta \cdot n^{z'-} \rceil$ and $f_\theta(\xbf_{[j]}^{z'-})$ denotes $j$-th largest scoring value over  the negative examples in group $z'$, i.e.  $  f_\theta ( \xbf_{[1]}^{z'-} )\geq  f_\theta( \xbf_{[2]}^{z'-})\geq  \ldots \geq f_\theta( \xbf_{[n_\beta^{z'-}]}^{z'-} )$.

 When the risk is posted by pAUC, we still face challenges in solving the above problem efficiently. The first challenges is posted by the ranking procedure in pAUC, which typically demands an additional $\Ocal(n^-\log(n^-))$ complexity to find the $n_\beta^-$-largest scores based on the negative sample. It has been shown that the ranking sum/average can be avoided by optimizing an auxiliary "threshold" parameter \citep{fan2017learning}. We summarize the result in the pAUC flavor in the following proposition.

\begin{proposition}\label{prop:pauc-equivalence}
Let $(a)_+ = \max\{0, a\}$ denote the ramp function at $0$. Then the nonnegative $\ell$-surrogated empirical risk of pAUC admits the following equivalent form
\[
\hat{R}_{z, z'}^\ell(\theta) \!=\! \min_{\rho_{z, z'} \geq 0} \Big\{\rho_{z, z'} + \frac{1}{n_\beta^{z'-}}\sum_{j=1}^{n^{z'-}}
\Big(\frac{1}{n^+}\sum_{i=1}^{n^{z+}} \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_j^{z'-})) - \rho_{z, z'}\Big)_+\Big\} \!\coloneqq\! \hat{R}_{z, z'}^\ell(\theta, \rho_{z, z'}).
\]
Moreover, $\rho \mapsto \hat{R}_{z, z'}^\ell(\,\cdot\,, \rho)$ is a convex function.
\end{proposition}
Since there are $k^2$ inter-group and intra-group in total, we require one $\rho_{z, z'}$ for each group. The problem in \eqref{eq:empirical-minimax-general} therefore becomes
\begin{equation}\label{eq:minimax-min}
\min_{\theta \in \Theta} \max_{\lambda \in \Lambda_{k^2}}\sum_{z=1}^{k} \sum_{z'=1}^{k}\lambda_{z, z'} \min_{\rho_{z, z'} \geq 0}\hat{R}^\ell_{z, z'}(\theta, \rho_{z, z'}).
\end{equation}
The above problem ruins the zero-sum game between $\theta$ and $\lambda$. Luckily, we can handle this second challenge by an equivalent zero-sum game as demonstrated in the following proposition. 

\begin{proposition}\label{prop:minimax-min-relaxed}
Denote $\rho = (\rho_{z, z'})_{z, z'=0}^{k-1}$. Then the problem \eqref{eq:minimax-min} is upper bounded, i.e.
\begin{equation}\label{eq:relaxed-pauc-obj}
\min_{\theta \in \Theta} \max_{\lambda \in \Lambda_{k^2}}\sum_{z=1}^{k} \sum_{z'=1}^{k}\lambda_{z, z'} \min_{\rho_{z, z'} \geq 0}\hat{R}^\ell_{z, z'}(\theta, \rho_{z, z'}) \leq \min_{\substack{\theta \in \Theta\\ \rho \succeq 0}} \max_{\lambda \in \Lambda_{k^2}} \lambda^\top \hat{R}^\ell(\theta, \rho; S).
\end{equation}
In particular, the two sides are equal if Assumption \ref{assmp:bounded-loss} holds.
\end{proposition}
The problem on the RHS of Eq. \eqref{eq:relaxed-pauc-obj} is a zero-sum game between the player $(\theta, \rho)$ and the player $\lambda$. We slightly abuse the notation and denote $\hat{R}^\ell(\theta, \rho, \lambda; S) = \lambda^\top \hat{R}^\ell(\theta, \rho; S)$. It serves as the objective as our proposed algorithm in the next section. 


\section{Proofs of Propositions\label{sec:proof-prop}}

\subsection{Proposition \ref{prop:pauc-equivalence}}

\begin{lemma}[\cite{fan2017learning}]\label{lem:top-k} 
Given a set of real numbers $\{a_1,\cdots,a_n\}$, its top-$k$ sum $\sum_{i=1}^k a_{[i]}$ is a convex function of $\{a_1,\cdots,a_n\}$. Moreover, $\sum_{i=1}^ka_{[i]}=\min_{\rho \geq 0}\{k\rho + \sum_{i=1}^n(a_i - \rho)_+\}$ if $a_i\geq0$ for any $i=1,\cdots,n$. The solution can be achieved when $\rho^* = a_{[k]}$.
\end{lemma}

\begin{proof}[Proof of Proposition Proposition \ref{prop:pauc-equivalence}]
Exchanging the double summation order in the $\ell$-surrogated pAUC risk gives
\begin{align*}
\widehat{\pauc}^\ell_{z, z'}(f) = & \frac{1}{n^{z+} n_\beta^{z'-}}
\sum_{i=1}^{n^{z+}} \sum_{j=1}^{n_\beta^{z'-}}  \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_{[j]}^{z'-})) \\
= & \frac{1}{n_\beta^{z'-}} \sum_{j=1}^{n_\beta^{z'-}} \Big(
\frac{1}{n^{z+}} \sum_{i=1}^{n^{z+}} \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_{[j]}^{z'-})) \Big) := \frac{1}{n_\beta^{z'-}} \sum_{j=1}^{n_\beta^{z'-}} s_{[j]}
\end{align*}
where $f_\theta(\xbf_{[j]}^{z'-})$ denotes $j$-th largest scoring value over the negative examples in group $z'$ and $s_j = \frac{1}{n^{z+}} \sum_{i=1}^{n^{z+}} \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_j^{z'-}))$ denotes the average score given $j$. Since the loss function $\ell$ is non-increasing, the score $s_{[j]}$ is also the $j$-largest score among $\{s_1, \cdots, s_{n^{z-}}\}$. Now calling Lemma \ref{lem:top-k} yields
\[
\hat{R}_{z, z'}^\ell(\theta) \!=\! \min_{\rho_{z, z'} \geq 0} \Big\{\rho_{z, z'} + \frac{1}{n_\beta^{z'-}}\sum_{j=1}^{n^{z'-}}
\Big(\frac{1}{n^+}\sum_{i=1}^{n^{z+}} \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_j^{z'-})) - \rho_{z, z'}\Big)_+\Big\} 
\]
Since $\Big(\frac{1}{n^+}\sum_{i=1}^{n^{z+}} \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_j^{z'-})) - \rho_{z, z'}\Big)_+$ is a piecewise linear function for any $j \in [n^{z'-}]$, and it is convex in $\rho$. The convexity in terms of $\rho$ follows by the sum of convex functions is still a convex function.
\end{proof}

\subsection{Proposition \ref{prop:minimax-min-relaxed}}

Since the minimization is a concave function, recalling the definition in Eq. \ref{eq:minimax-min}, we have 
\[
\sum_{z=1}^{k} \sum_{z'=1}^{k}\lambda_{z, z'} \min_{\rho_{z, z'} \geq 0}\hat{R}^\ell_{z, z'}(\theta, \rho_{z, z'}) = \min_{\rho \succeq 0}\sum_{z=1}^{k} \sum_{z'=1}^{k}\lambda_{z, z'} \hat{R}^\ell_{z, z'}(\theta, \rho_{z, z'}) = \min_{\rho \succeq 0} \lambda^\top \hat{R}^\ell(\theta, \rho).
\]
For any $\theta \in \Theta$, $\rho \in [0, \infty)^{k^2}$ and $\lambda \in \Lambda_{k^2}$, we have 
\[
\min_{\rho \succeq 0}\lambda^\top \hat{R}^\ell(\theta, \rho) \leq \lambda^\top \hat{R}^\ell(\theta, \rho)
\]
which implies for any $\theta \in \Theta$ and $\rho \in [0, \infty)^{k^2}$
\[
\max_{\lambda \in \Lambda_{k^2}}\min_{\rho \succeq 0}\lambda^\top \hat{R}^\ell(\theta, \rho) \leq \max_{\lambda \in \Lambda_{k^2}}\lambda^\top \hat{R}^\ell(\theta, \rho).
\]
Taking the minimum over $\rho$ yields for any $\theta \in \Theta$
\begin{equation}\label{eq:max-min}
\max_{\lambda \in \Lambda_{k^2}}\min_{\rho \succeq 0}\lambda^\top \hat{R}^\ell(\theta, \rho) \leq \min_{\rho \succeq 0}\max_{\lambda \in \Lambda_{k^2}}\lambda^\top \hat{R}^\ell(\theta, \rho).
\end{equation}
The first part of the proposition follows by taking the minimum over $\theta$ on both sides. Since $\rho_{z, z'}^* = \frac{1}{n^{z+}} \sum_{i=1}^{n^{z+}} \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_[n_\beta^{z'-}]^{z'-}))$ is always a solution by Lemma \ref{lem:top-k} for any $z, z' \in \Zcal$. If Assumption \ref{assmp:bounded-loss} holds, then $\rho_{z, z'}^* \leq M$ for any $z, z' \in \Zcal$. Therefore \eqref{eq:max-min} becomes
\[
\max_{\lambda \in \Lambda_{k^2}}\min_{\rho \in [0, M]^{k^2}}\lambda^\top \hat{R}^\ell(\theta, \rho) \leq \min_{\rho  \in [0, M]^{k^2}}\max_{\lambda \in \Lambda_{k^2}}\lambda^\top \hat{R}^\ell(\theta, \rho).
\]
Since $(\lambda, \rho) \mapsto \lambda^\top \hat{R}^\ell(\theta, \rho)$ is convex in $\rho$ and concave in $\lambda$, while $\Lambda_{k^2}$ and $[0, M]^{k^2}$ are both compact convex sets, the equaility holds by the Von Neumann's minimax theorem \cite{von2007theory}. Taking the minimum over $\theta$ on both sides yields the desired result.


In this section, We focus on the case that the fairness risk is posted by group-level pAUC. The results for AUC-based objective can be found in Appendix \ref{sec:auc}. We aim to develop a SGDA-type algorithm (e.g. \cite{nemirovski2009robust}) to solve \eqref{eq:relaxed-pauc-obj}. 
% To this end, we rewrite the objective as
% \[
% \hat{R}^\ell(\theta, \rho, \lambda; S) = \sum_{z=1}^{k}\sum_{z'=1}^{k}\lambda_{z,z'}\Big(\frac{1}{n^{z-}}\sum_{j=1}^{n^{z-}} 
% \]
\begin{algorithm}[ht!]
\caption{Stochastic Min-max Algorithm for Fair pAUC\label{alg:mm-fair-pauc}}
\begin{algorithmic}[1]
\STATE {\bf Inputs:} Number of iterations $T$, batch size $m$, step sizes $\{\eta_t\}_{t=1}^T$ and $p_{z, z'} = \frac{n^{z+} + n^{z'-}}{\sum_{z,z'} (n^{z+} + n^{z'-})}$
\STATE {Initialize $\theta_0 \in \Theta$, $\rho_0 \in [0, \infty)^{k^2}$ and $\lambda_0 = (p_{z, z'})_{z, z'=0}^{k-1}$}
\FOR{$t=1$ to $T$}
\STATE{$B_t = \texttt{Sample}_m(S)$}
\STATE{$\begin{pmatrix}\theta_t\\ \rho_t\end{pmatrix} = \texttt{Proj}_{\Theta\times [0, \infty)^{k^2}}\Big(\begin{pmatrix}\theta_{t-1}\\ \rho_{t-1}\end{pmatrix} -\eta_t \begin{pmatrix}\lambda_{t-1}^\top\partial_\theta\hat{R}^\ell(\theta_{t-1}, \rho_{t-1}; B_t) \\ \lambda_{t-1}^\top\partial_\rho\hat{R}^\ell(h_{t-1}, \rho_{t-1}; B_t)\end{pmatrix}\Big)$}
\STATE{$\lambda_t = \texttt{Proj}_{\Lambda_{k^2}}(\lambda_{t-1} + \eta_t \hat{R}^\ell(\theta_{t-1}, \rho_{t-1}; B_t))$}
\ENDFOR
\STATE {\bf Outputs:} $\theta_T$
\end{algorithmic}
\end{algorithm}

\begin{lemma}
The update $\lambda_t$ by solving the regularized problem by $D_\Phi(\cdot \parallel \lambda_{t-1})$, i.e.
\begin{align*}
\lambda_t = & \arg\max_{\lambda \in \Lambda_{k^2}}  \eta_t\lambda_{t-1}^\top \hat{R}^\ell(\theta_{t-1}; B_t) + \eta_t(\lambda - \lambda_{t-1})^\top \hat{R}^\ell(\theta_{t-1}; B_t) - D_\Phi(\lambda \parallel \lambda_{t-1}) \\
= & \arg\max_{\lambda \in \Lambda_{k^2}} \eta_t\lambda^\top \hat{R}^\ell(\theta_{t-1}; B_t) - D_\Phi(\lambda \parallel \lambda_{t-1}) 
\end{align*}
is equivalent to mirror descent, i.e.
\[
\lambda_t = \frac{\lambda_{t-1}\exp(\eta_t \hat{R}^\ell(\theta_{t-1}; B_t))}{\|\lambda_{t-1}\exp(\eta_t \hat{R}^\ell(\theta_{t-1}; B_t))\|_1}.
\]
\end{lemma}



\begin{lemma}
The update $\lambda_t$ by solving the regularized problem by $\Phi$ is identical as follow
\begin{align*}
\lambda_t = & \arg\max_{\lambda \in \Lambda_{k^2}} \eta_t\lambda^\top \hat{R}^\ell(\theta_{t-1}; B_t) - \Phi(\lambda) \\
= & \frac{\exp(\eta_t \hat{R}^\ell(\theta_{t-1}; B_t))}{\|\exp(\eta_t \hat{R}^\ell(\theta_{t-1}; B_t))\|_1},
\end{align*}
and the problem is equivalent to the log-sum-exp
\[\max_{\lambda \in \Lambda_{k^2}} \eta_t\lambda^\top \hat{R}^\ell(\theta_{t-1}; B_t) - \Phi(\lambda) = \log(\sum_{z=0}^{k-1}\sum_{z=0}^{k-1} \exp(\eta_t \hat{R}_{z, z'}^\ell(\theta_{t-1}; B_t))).\]
\end{lemma}

\begin{lemma}
Let $\eta_t = \eta$. The update $\lambda_t$ by mirror descent is identical as the following regularized problem
\[
\lambda_t = \arg\max_{\lambda \in \Lambda_{k^2}} \eta \sum_{\tau=1}^{t-1} \lambda^\top \hat{R}^\ell(\theta_\tau; B_{\tau+1}) - \Phi(\lambda)
\]
\end{lemma}

\begin{proof}
First, observe that the unconstrained maximum
\[
\lambda^* = \arg\max_{\lambda} \eta \sum_{\tau=1}^{t-1} \lambda^\top \hat{R}^\ell(\theta_\tau; B_{\tau+1}) - \Phi(\lambda)
\]
satisfies
\[\nabla \Phi(\lambda^*) = \eta \sum_{\tau=1}^{t-1} \hat{R}^\ell(\theta_\tau; B_{\tau+1}).\]
By definition, $\gamma_t$ also satisfies the above equation, but since $\Phi$ is strongly convex, there is only one solution for the above equation and thus $\gamma_t = \lambda^*$. Hence,
\begin{align*}
D_\Phi(\lambda \parallel \gamma_t) = & \Phi(\lambda) - \Phi(\gamma_t) - \nabla\Phi(\gamma_t)^\top(\lambda - \gamma_t)  \\
= & \Phi(\lambda) - \Phi(\gamma_t) - \eta \sum_{\tau=1}^{t-1} \hat{R}^\ell(\theta_\tau; B_{\tau+1})^\top(\lambda - \gamma_t).
\end{align*}
Since $\Phi(\gamma_t)$ and $\sum_{\tau=1}^{t-1} \hat{R}^\ell(\theta_\tau; B_{\tau+1})^\top\gamma_t$ are independent of $\lambda$, it follows that $D_\Phi(\lambda \parallel \gamma_t)$ is minimized at the point $\lambda$ that minimizes $\Phi(\lambda) - \eta \sum_{\tau=1}^{t-1} \hat{R}^\ell(\theta_\tau; B_{\tau+1})^\top\lambda$ over $\Lambda_{k^2}$ which, in turn, implies that
\[\arg\min_{\lambda \in \Lambda_{k^2}} D_\Phi(\lambda \parallel \gamma_t) = \arg\min \Phi(\lambda) - \eta \sum_{\tau=1}^{t-1} \hat{R}^\ell(\theta_\tau; B_{\tau+1})^\top\lambda.\]
\end{proof}

We first focus on the convex-concave case. The proof is inspired by \cite{nemirovski2009robust}. We first prove the generalized Pythagorean Theorem.


\begin{lemma}\label{lem:pythagorean}
Let $\Lambda$ be a convex set. Suppose $L$ is a proper convex function whose domain containing $\Lambda$. Let $\lambda$ be the projection of $\lambda'$ onto $\Lambda$, i.e.
\[\lambda^\star = \arg\min_{\lambda \in \Lambda} L(\lambda) + D_\Phi(\lambda\parallel\lambda'),\]
then for any $\gamma \in \Lambda$ we have
\[L(\lambda^\star) + D_\Phi(\gamma\parallel\lambda^\star) + D_\Phi(\lambda^\star\parallel\lambda') \leq L(\gamma) + D_\Phi(\gamma\parallel\lambda')\]
\end{lemma}

\begin{proof}
Since $\nabla_\lambda D_\Phi(\lambda\parallel\lambda') = \nabla \Phi(\lambda) - \nabla \Phi(\lambda')$, by the first-order optimality at $\lambda^\star$, we have for any $\gamma \in \Lambda$ that
\[(\nabla L(\lambda^\star) + \nabla \Phi(\lambda^\star) - \nabla \Phi(\lambda'))^\top (\gamma - \lambda^\star) \geq 0.\]
Since $L$ is convex, we have for any $\gamma \in \Lambda$ that
\begin{align*}
L(\gamma) \geq & L(\lambda^\star) + \nabla L(\lambda^\star)^\top (\gamma - \lambda^\star) \\
\geq & L(\lambda^\star) + (\nabla \Phi(\lambda') - \nabla \Phi(\lambda^\star))^\top (\gamma - \lambda^\star) \\
= & L(\lambda^\star) - \nabla \Phi(\lambda^\star)^\top (\lambda^\star - \lambda') + \Phi(\lambda^\star) - \Phi(\lambda') \\
& + \nabla \Phi(\lambda')^\top (\gamma - \lambda') + \Phi(\gamma) - \Phi(\lambda') \\
& - \nabla \Phi(\lambda^\star)^\top (\gamma - \lambda^\star) + \Phi(\gamma) - \Phi(\lambda^\star) \\
= & L(\lambda^\star) + D_\Phi(\lambda^\star\parallel\lambda') - D_\Phi(\gamma\parallel\lambda') + D_\Phi(\gamma\parallel\lambda^\star).
\end{align*}
Rearranging completes the proof.
\end{proof}

\begin{lemma}\label{lem:first-order-convergence}
The following inequality holds
\[\Ebb\Big[\max_{\omega\in \Omega}\sum_{t=1}^T \eta_t \nabla \hat{R}(\omega_{t-1}; S)^\top (\omega_{t-1} - \omega)\Big] \leq  1 + \frac{G^2}{2} \sum_{t=1}^T  \eta_t^2 + 2G \sqrt{\sum_{t=1}^T \eta_t^2}\]
\end{lemma}

\begin{proof}
Considering $L(\omega) = \eta_t \nabla \hat{R}(\omega_{t-1}; B_t)^\top (\omega - \omega_{t-1})$ in Lemma \ref{lem:pythagorean} and rearranging, we have
\begin{align*}
\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)^\top (\omega_{t-1} - \omega) 
\leq & \eta_t \nabla \hat{R}(\omega_{t-1}; B_t)^\top (\omega_t - \omega_{t-1}) + D_\Pi(\omega\parallel\omega_{t-1}) - D_\Pi(\omega\parallel\omega_t)\\
& - D_\Pi(\omega_t\parallel\omega_{t-1}).
\end{align*}
Since $\Pi$ is $1$-strongly convex with respect to the norm $\|\cdot\|$, it is straightforward to check $D_\Pi(\omega_t\parallel\omega_{t-1}) \geq \frac{1}{2}\|\omega_t - \omega_{t-1}\|^2$. Together with Young's inequality, we further derive
\begin{align*}
\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)^\top (\omega_{t-1} - \omega) \leq & \frac{1}{2}\|\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)\|_*^2 + \frac{1}{2}\|\omega_t - \omega_{t-1}\|^2 \\
& + D_\Pi(\omega\parallel\omega_{t-1}) - D_\Pi(\omega\parallel\omega_t) - D_\Pi(\omega\parallel\omega_t)\\
\leq & \frac{1}{2}\|\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)\|_*^2 + \frac{1}{2}\|\omega_t - \omega_{t-1}\|^2\\
&  + D_\Pi(\omega\parallel\omega_{t-1}) - D_\Pi(\omega\parallel\omega_t) - \frac{1}{2}\|\omega_t - \omega_{t-1}\|^2\\
= & \frac{1}{2}\|\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)\|_*^2 + D_\Pi(\omega\parallel\omega_{t-1}) - D_\Pi(\omega\parallel\omega_t).
\end{align*}
This relation implies that for every $\omega \in \Omega$, we have
\begin{align*}
\eta_t \nabla \hat{R}(\omega_{t-1}; S)^\top (\omega_{t-1} - \omega) \leq & \frac{1}{2}\|\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)\|_*^2 + D_\Pi(\omega\parallel\omega_{t-1}) - D_\Pi(\omega\parallel\omega_t)\\
& - \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) - \nabla \hat{R}(\omega_{t-1}; S))^\top (\omega_{t-1} - \omega).
\end{align*}
Summing up these inequalities over $t=1, \cdots, T$ we arrive
\begin{align*}
\sum_{t=1}^T \eta_t \nabla \hat{R}(\omega_{t-1}; S)^\top (\omega_{t-1} - \omega) \leq &  D_\Pi(\omega\parallel\omega_0) - D_\Pi(\omega\parallel\omega_T) + \sum_{t=1}^T \frac{1}{2}\|\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)\|_*^2\\
& - \sum_{t=1}^T \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) - \nabla \hat{R}(\omega_{t-1}; S))^\top (\omega_{t-1} - \omega)\\
\leq & D_\Pi(\omega\parallel\omega_0)  + \sum_{t=1}^T \frac{1}{2}\|\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)\|_*^2 \\
& - \sum_{t=1}^T \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) - \nabla \hat{R}(\omega_{t-1}; S))^\top (\omega_{t-1} - \omega) \\
\leq & D_\Pi(\omega\parallel\omega_0)  + \sum_{t=1}^T \frac{1}{2}\|\eta_t \nabla \hat{R}(\omega_{t-1}; B_t)\|_*^2 \\
& + \Big\|\sum_{t=1}^T \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) - \nabla \hat{R}(\omega_{t-1}; S))\Big\|_* \|\omega\| \\
& - \sum_{t=1}^T \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) - \nabla \hat{R}(\omega_{t-1}; S))^\top \omega_{t-1} 
\end{align*}
where we used $D_\Pi(\omega\parallel\omega') \geq 0$ for any $\omega, \omega'$ in the second inequality, and we used the Cauchy-Schwarz inequality in the last one. Since $\omega_{t-1}$ is deterministic functions given $B_1, \cdots, B_t$, we conclude that $\Ebb[(\nabla \hat{R}(\omega_{t-1}; B_t) - \nabla \hat{R}(\omega_{t-1}; S))^\top \omega_{t-1}] = 0$ by the tower rule. On the other hand, by the Jensen's inequality and the tower rule, we know
\begin{align*}
\Big(\Ebb\Big\|\sum_{t=1}^T \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) \!-\! \nabla \hat{R}(\omega_{t-1}; S))\Big\|_*\Big)^2 \leq & \Ebb\Big[\Big\|\sum_{t=1}^T \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) \!-\! \nabla \hat{R}(\omega_{t-1}; S))\Big\|_*^2\Big] \\
= & \sum_{t=1}^T \Ebb\Big[\Big\| \eta_t (\nabla \hat{R}(\omega_{t-1}; B_t) \!-\! \nabla \hat{R}(\omega_{t-1}; S))\Big\|_*^2\Big] \\
\leq & 4 G^2\sum_{t=1}^T \eta_t^2.
\end{align*}
Now, since the above inequality holds for all $\omega$, we take expectation and get
\begin{align*}
\Ebb\Big[\max_{\omega\in \Omega}\sum_{t=1}^T \eta_t \nabla \hat{R}(\omega_{t-1}; S)^\top (\omega_{t-1} - \omega)\Big] \leq & \max_{\omega\in \Omega} D_\Pi(\omega\parallel\omega_0) + \frac{G^2}{2} \sum_{t=1}^T  \eta_t^2 + 4G^2 \sqrt{\sum_{t=1}^T \eta_t^2}
\end{align*}
Since $\omega_0 \in \arg\min_{\omega \in\Omega} \Pi(\omega)$, it follows that
\begin{align*}
\Ebb\Big[\max_{\omega\in \Omega}\sum_{t=1}^T \eta_t \nabla \hat{R}(\omega_{t-1}; S)^\top (\omega_{t-1} - \omega)\Big] \leq & 1 + \frac{G^2}{2} \sum_{t=1}^T  \eta_t^2 + 2G \sqrt{\sum_{t=1}^T \eta_t^2}
\end{align*}
\end{proof}

\begin{theorem}
Assume Assumption \ref{assmp:bounded-domain}, \ref{assmp:bounded-loss} \ref{assmp:lipschitz-continuity} and \ref{assmp:bounded-variance} hold. Assume the scoring function $f$ is linear. The updates $\{\theta_t, \lambda_t\}_{t=1}^T$ of Algorithm \ref{alg:mm-fair-auc} satisfies the following inequalities
\begin{enumerate}[label=\alph*)]
\item For a fixed number $T$, if $\eta_t = \eta = \frac{2c}{3G\sqrt{T}}$, we have
\[\Ebb[\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_T, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_T)] \leq \max\{c, c^{-1}\}\frac{2G}{\sqrt{T}}. \]
\item Let $\eta_t = \frac{cD}{G\sqrt{t}}$, we have
\begin{align*}
\Ebb[\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_{T_0:T}, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_{T_0:T})] \leq (\max\{c, c^{-1}\} + 1) \frac{2DGC(r)}{\sqrt{T}}.
\end{align*}
\end{enumerate}
\end{theorem}

\begin{proof}
We use the notation $\omega = (\theta, \lambda)$ and equip $\Rbb^d \times \Rbb^{k^2}$ with norm 
\[\|\omega\| = \sqrt{\frac{1}{2D^2}\|\theta\|_2^2 + \frac{1}{2\log (k^2)} \|\lambda\|_1^2},\]
so that the dual norm is 
\[\|\omega\|_* = \sqrt{2D^2\|\theta\|_2^2 + 2\log (k^2) \|\lambda\|_\infty^2},\]
and set 
\[G^2 = 2D_\theta^2 G_\theta^2 + 2\log (k^2) M^2.\]
We equip the set $\Omega = \Theta \times \Lambda_{k^2}$ with the mirror map $\Pi$ such that
\[\Pi(\omega) = \frac{1}{2D^2}\Psi(\theta) + \frac{1}{2\log (k^2)} \Phi(\lambda).\]
It is immediately seen that $\Pi$ is indeed a mirror map for $\omega \in \Omega$ with respect to the norm $\|\cdot\|$. We can therefore define the Bregman divergence and the proximal mapping with respect to $\Pi$ and the observe Line 5-7 in Algorithm \ref{alg:rmw-fair-auc} is the mirror-descent with respect to $\omega$. By convexity of $\hat{R}^\ell(\cdot, \lambda)$, we have
\[\hat{R}^\ell(\theta_t, \lambda_t) - \hat{R}^\ell(\theta, \lambda_t) \leq (\theta_t - \theta)^\top \partial_\theta \hat{R}^\ell(\theta_t, \lambda_t),\]
for any $\theta \in \Theta$. And by the concavity
\[\hat{R}^\ell(\theta_t, \lambda) - \hat{R}^\ell(\theta_t, \lambda_t) \leq (\lambda - \lambda_t)^\top \partial_\lambda \hat{R}^\ell(\theta_t, \lambda_t),\]
so that for all $\omega = \theta \times \lambda$,
\[\hat{R}^\ell(\theta_t, \lambda) - \hat{R}^\ell(\theta, \lambda_t) \leq (\theta_t - \theta)^\top \partial_\theta \hat{R}^\ell(\theta_t, \lambda_t) + (\lambda - \lambda_t)^\top \partial_\lambda \hat{R}^\ell(\theta_t, \lambda_t) = (\omega_t - \omega)^\top \nabla \hat{R}^\ell(\omega_t).\]
Using once again the convexity-concavity of $R$, we write
\begin{align*}
\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_T, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_T) \leq & \Big(\sum_{t=1}^T \eta_t\Big)^{-1}    \Big(\max_{\lambda \in \Lambda_{k^2}} \sum_{t=1}^T \eta_t\hat{R}^\ell(\theta_t, \lambda) - \min_{\theta \in \Theta} \sum_{t=1}^T \eta_t\hat{R}^\ell(\theta, \lambda_t)\Big)  \\
\leq & \Big(\sum_{t=1}^T \eta_t\Big)^{-1}  \max_{\omega \in \Omega} \sum_{t=1}^T \eta_t (\omega_t - \omega)^\top\nabla \hat{R}^\ell(\omega_t).
\end{align*}
By Lemma \ref{lem:first-order-convergence}, taking expectation on both sides we derive
\begin{align*}
\Ebb[\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_T, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_T)] \leq & \Big(\sum_{t=1}^T \eta_t\Big)^{-1}\Big(1 + \frac{G^2}{2} \sum_{t=1}^T  \eta_t^2 + 2G \sqrt{\sum_{t=1}^T \eta_t^2}\Big).
\end{align*}
For a fixed number of $T$, and constant stepsize policy $\eta_t = \eta = \frac{2c}{3G \sqrt{T}}$, we have
\[\Ebb[\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_T, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_T)] \leq \max\{c, c^{-1}\}\frac{2G}{\sqrt{T}}, \]
which proves Part a). To prove Part b), we denote
\begin{align*}
D = & \sqrt{2} \Big(\sup_{\omega, \omega' \in \Omega} D_\Pi(\omega\parallel\omega')\Big)^{1/2}\\
= &\sqrt{2} \Big(\sup_{\omega, \omega' \in \Omega} \Pi(\omega) - \Pi(\omega') - (\omega - \omega')^\top \nabla\Pi(\omega')\Big)^{1/2},
\end{align*}
and assume it is finite. The proof above shows that for any $1 < T_0 \leq T$, we have
\begin{align*}
& \Ebb[\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_{T_0:T}, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_{T_0:T})] \\
\leq & \Big(\sum_{t=T_0}^T \eta_t\Big)^{-1}\Big(\sup_{\omega, \omega' \in \Omega} D_\Pi(\omega\parallel\omega') + \frac{G^2}{2} \sum_{t=T_0}^T  \eta_t^2 + 2G \sqrt{\sum_{t=T_0}^T \eta_t^2}\Big)\\
\leq & \Big(\sum_{t=T_0}^T \eta_t\Big)^{-1}\Big(D^2 + \frac{G^2}{2} \sum_{t=T_0}^T  \eta_t^2 + 2G \sqrt{\sum_{t=T_0}^T \eta_t^2}\Big).
\end{align*}
Consider variable stepsizes $\eta_t = \frac{cD}{G\sqrt{t}}$, we have
\begin{align*}
\Ebb[\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_{T_0:T}, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_{T_0:T})] \leq \frac{DG}{\sqrt{T}}\Big(\frac{1}{c} \frac{T}{T - T_0 + 1} + \frac{c}{2}\frac{T}{T_0} + 2\frac{T}{\sqrt{T_0(T-T_0+1)}}\Big).
\end{align*}
Therefore when $T_0 = \lceil rT\rceil$ we have
\begin{align*}
\Ebb[\max_{\lambda \in \Lambda_{k^2}} \hat{R}^\ell(\tilde{\theta}_{T_0:T}, \lambda) - \min_{\theta \in \Theta} \hat{R}^\ell(\theta, \tilde{\lambda}_{T_0:T})] \leq (\max\{c, c^{-1}\} + 1) \frac{2DGC(r)}{\sqrt{T}}.
\end{align*}
The proof is complete.
\end{proof}


\section{Results for AUC-based objectives \label{sec:auc}}
In this section, we present the algorithm and analysis when the group-level risk is posted by inter-group and intra-group AUC. The objective is given by
\[
\min_{\theta \in \Theta} \max_{\lambda \in \Lambda_{k^2}} \sum_{z=1}^{k} \sum_{z'=1}^{k} \lambda_{z, z'} \hat{R}^\ell_{z, z'}(\theta) = \sum_{z=1}^{k} \sum_{z'=1}^{k}  \frac{\lambda_{z, z'}}{n^{z+}n^{z'-}}\sum_{i=1}^{n^{z+}}\sum_{j=1}^{n^{z'-}} \ell(f_\theta(\xbf_i^{z+}) - f_\theta(\xbf_j^{z'-})) \coloneqq \hat{R}^\ell(\theta, \lambda; S).
\]
We are now at the position of presenting our algorithm for this problem.

\begin{algorithm}[ht!]
\caption{Stochastic Gradient Descent Ascent for Fair AUC\label{alg:mm-fair-auc}}
\begin{algorithmic}[1]
\STATE {\bf Inputs:} Number of iterations $T$, batch size $m$, step sizes $\{\eta_t\}_{t=1}^T$ and $p_{z, z'} = \frac{n^{z+} + n^{z'-}}{\sum_{z,y} n^{zy}}$
\STATE {Initialize $\theta_0 \in \Theta$ and $\lambda_0 = (p_{z, z'})_{z, z'=0}^{k-1}$}
\FOR{$t=1$ to $T$}
\STATE{$B_t = \texttt{Sample}_m(S)$}
\STATE{$\theta_t = \texttt{Proj}_\Theta(\theta_{t-1} -\eta_t \partial_\theta\hat{R}^\ell(\theta_{t-1}, \lambda_{t-1}; B_t))$}
\STATE{$\lambda_t = \texttt{Proj}_{\Lambda_{k^2}}(\lambda_{t-1} + \eta_t \partial_\lambda\hat{R}^\ell(\theta_{t-1}, \lambda_{t-1}; B_t))$}
\ENDFOR
\STATE {\bf Outputs:} $\theta_T$
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:mm-fair-auc} is inspired by the classical SGDA algorithm \cite{nemirovski2009robust} for efficient computation on large datasets, which simultaneously update the min-player and the max-player based on the same batch of stochastic gradients. Here we highlight the differences between our designed Algorithm \ref{alg:mm-fair-auc} and genetic SGDA.


